Towards Probabilistic Session-Type Monitoring

We present a tool-based approach for the runtime analysis of communicating processes grounded on probabilistic binary session types. We synthesise a monitor out of a probabilistic session type where each choice point is decorated by a probability distribution. The monitor observes the execution of a process, infers its probabilistic behaviour and issues warnings when the observed behaviour deviates from the one specified by the probabilistic session type.

==> Makefile <==
PROJECT=main
TEX=pdflatex
BIBTEX=bibtex
BUILDTEX=$(TEX) $(PROJECT).tex

all:
	$(BUILDTEX)
	$(BIBTEX) $(PROJECT)
	$(BUILDTEX)
	$(BUILDTEX)
	# rm -f *.log *.bak *.aux *.bbl *.blg *.idx *.toc *.out *.gz *.pdfsync *.lof *~
	detex main.tex | wc -w

clean:
	find . -name "*~" -exec rm -rf {} \;
	find . -name "*.log" -exec rm -rf {} \;
	find . -name "*.aux" -exec rm -rf {} \;
	find . -name "*.out" -exec rm -rf {} \;
	find . -name "*.synctex.gz" -exec rm -rf {} \;
	find . -name "*.bbl" -exec rm -rf {} \;
	find . -name "*.blg" -exec rm -rf {} \;
	find . -name "*.fdb*" -exec rm -rf {} \;
	find . -name "*.fls*" -exec rm -rf {} \;

